A Research Roadmap for Augmenting Software Engineering Processes and Software Products with Generative AI

Generative AI (GenAI) is rapidly transforming software engineering (SE) practices, influencing how SE processes are executed, as well as how software systems are developed, operated, and evolved. This paper applies design science research to build a roadmap for GenAI-augmented SE. The process consists of three cycles that incrementally integrate multiple sources of evidence, including collaborative discussions from the FSE 2025 "Software Engineering 2030" workshop, rapid literature reviews, and external feedback sessions involving peers. McLuhan's tetrads were used as a conceptual instrument to systematically capture the transforming effects of GenAI on SE processes and software products. The resulting roadmap identifies four fundamental forms of GenAI augmentation in SE and systematically characterizes their related research challenges and opportunities. These insights are then consolidated into a set of future research directions. By grounding the roadmap in a rigorous multi-cycle process and cross-validating it among independent author teams and peers, the study provides a transparent and reproducible foundation for analyzing how GenAI affects SE processes, methods and tools, and for framing future research within this rapidly evolving area.

==> comments.tex <==
\begin{comment}  
Sauvola et al. \cite{10.1007/s10515-024-00426-z} identify improvements to code comprehension, debugging, testing, deployment, and maintenance through automated capabilities and faster feedback loops.
Similarly, Kam et al. \cite{10.1145/3696630.3727251} and Banh et al. \cite{10.1016/j.infsof.2025.107751} describe productivity increases during conceptualization, code analysis, refinement, and error identification.
These enhancements not only accelerate development time but also improve developer experience by reducing context-switching and cognitive overhead.

Hou et al. \cite{10.1145/3695988} provide quantitative evidence, with most LLM applications enhancing mid-phase SDLC tasks: coding (57\%), maintenance (23\%), and quality assurance (15\%).
Wang et al.\cite{WangHCLWW24} echo this in the domain of software testing, with LLMs improving test generation, bug detection, program repair, and debugging, leading to faster testing cycles and increased coverage.

Enhancements are not restricted to core engineering tasks:
Rico and Öberg \cite{10.1145/3696630.3728718} discuss improvements in effort estimation, requirements refinement, stakeholder-aware documentation, and team training.
Qiu et al. \cite{10.1145/3709353} also include mental health monitoring, personalized learning, and improved team coordination, forecasting broader impact on productivity and well-being. Guimaraes and Nascimento \cite{10.1145/3696630.3730538} and Terragni et al. \cite{10.1145/3715003} position AI as a central enabler across implementation, architecture, and development workflows.

In summary, several critical areas exemplify the enhancement:
First, \textit{Requirements Engineering} is significantly amplified through improved extraction, analysis, and validation techniques, allowing for richer elicitation and clearer communication of stakeholder needs (Ferrari and Spoletini~\cite{10.1016/j.infsof.2025.107697}).
Second, \textit{Automated Design and Documentation} practices benefit from the generation of context-sensitive and stakeholder-specific artefacts, thereby reducing manual workload and ensuring that design intent is preserved throughout project iterations (Rico and Öberg~\cite{10.1145/3696630.3728718}).
Furthermore, \textit{Testing and Debugging} are enhanced by intelligent test case generation and automated program repair, which can vastly accelerate the fault localization and correction processes (Wang et al.~\cite{WangHCLWW24}).
\textit{Code Quality and Review} workflows also gain precision through the automatic identification of errors and real-time quality assurance feedback, enabling developers to maintain higher standards of software robustness and maintainability (Kam et al.~\cite{10.1145/3696630.3727251}; Lyu et al.~\cite{10.1145/3708519}).
Lastly, \textit{Developer Support} is significantly elevated, especially in areas such as onboarding, learning, and prototyping, where intelligent assistants provide tailored documentation, examples, and code suggestions to accelerate skill acquisition and reduce cognitive overhead (Qiu et al.~\cite{10.1145/3709353}; Keim et al.~\cite{keim_automated_2025}).
Collectively, these enhancements underscore how AI technologies act as amplifiers within the software engineering ecosystem, reshaping traditional workflows and augmenting human capabilities.
\end{comment}
\begin{comment}
    

Storey et al. \cite{10.1145/3678172} and Hou et al. \cite{10.1145/3695988} assert that the traditional need for manually created documentation and code search is reduced or disappears.
Wang et al. \cite{WangHCLWW24} and Qiu et al. \cite{10.1145/3709353} highlight that test generation, bug reproduction, and oracle design are increasingly AI-supported, replacing laborious manual processes.

Ferrari and Spoletini \cite{10.1016/j.infsof.2025.107697} predict that the exclusive domain of formal methods experts may diminish, and routine elicitation tasks performed by dedicated requirements engineers may become automated, an idea echoed by Terragni et al. \cite{10.1145/3715003}.
Likewise, Lyu et al. \cite{10.1145/3708519} position the developer more as a reviewer or quality specialist than a traditional code writer.

To conclude, several once-central tasks are increasingly displaced by automated alternatives.
\textit{Manual Requirements Elicitation and Formalization}, traditionally involving labor-intensive stakeholder interviews and structured documentation, are now supplemented by AI-mediated extraction from conversational artifacts such as emails or meeting transcripts, streamlining specification without direct manual intervention (Ferrari and Spoletini~\cite{10.1016/j.infsof.2025.107697}; Terragni et al.~\cite{10.1145/3715003}).
Similarly, \textit{Manual Testing and Debugging}, longstanding components of the software lifecycle, are being replaced by automated tools that offer predictive test generation, bug localization, and patch suggestions with minimal human oversight (Wang et al.~\cite{WangHCLWW24}).
The once-common task of \textit{Code Snippet Search}, a staple of developer workflows, is also diminished due to the rise of prompt-driven, context-aware code synthesis, reducing dependence on external sources like Stack Overflow (Storey et al.~\cite{10.1145/3678172}).
In parallel, the laborious writing of \textit{Developer Documentation} is giving way to real-time generation of stakeholder-specific and usage-sensitive documentation, embedded directly into development environments (Rico and Öberg~\cite{10.1145/3696630.3728718}).
Lastly, \textit{Hand-written Workflows and Quality Assurance (QA) Steps} are increasingly automated through program repair systems and continuous quality feedback mechanisms, which reduce the need for manually orchestrated test and deployment procedures (Guimaraes and Nascimento~\cite{10.1145/3696630.3730538}).
Collectively, these obsolescences underscore the reconfiguration of software engineering labor, wherein AI automates routine tasks, allowing developers to focus more on high-level reasoning and system design.

\end{comment}

\begin{comment}
    A discussion with participants of the Requirements Engineering conference 2025 (RE2025) also resulted in the following ideas\pat{didn't find this on the research methodology. It comes out of the blue.}:
\begin{itemize}
    \item Requirements engineering gets more important than ever, if they are regarded as the input on which the following steps are (semi-) automatically performed.
    \item There can be the ability to scale requirements elicitation to many stakeholders, without additional costs, by performing the interviews with LLMs.
    \item There might be the possibility to check the consistency of requirements and other artifacts with automated formalization \marco{This last part of the sentence should also be checked }  and integrating formal verifiers early.
\end{itemize}
\end{comment}

\begin{comment}
    \subsection{Validity Risks}
\label{sec:validity1}
\pat{it should be useful to have risks discussed in just one place. Now they are discusses all around the paper. We can instead have a subsection of the research method or a section at the end of the paper.}
This Rapid Literature Review presents some validity threats by its design.
\paragraph{Construct validity} Our search string might not have captured all relevant literature, which could have limited the breadth of our study. 
Furthermore, the use of LLM-based filtering may have inadvertently removed relevant publications, leading to incomplete coverage. 
To reduce this threat, we manually inspected samples of the excluded papers to validate the filtering process.

\paragraph{External validity} The selection of specific conferences and journals may bias our results, as relevant discussions—particularly those concerning future directions—may also appear in other venues such as workshops or seminars that our search strategy did not include.
We mitigated this by choosing the top-tier software engineering conferences and journals, ensuring that our dataset at least covers the main outlets where influential research is typically published.

\paragraph{Internal validity} In several cases, we had to interpret and consolidate statements with varying wordings from different authors. This process may have introduced risks of misinterpretation or misunderstanding, potentially influencing the outcomes of our analysis.
%\begin{itemize}
%    \item Our search string might miss relevant literature;
%    \item The filtering using LLMs might have removed relevant literature, making our results incomplete;
%    \item Our focus on certain conferences and journals might affect the outcome. Discussions about the future might also be present in other venues like dedicated workshops or seminars that our search strategy did not include;
%    \item Sometimes, we had to interpret statements and map different wordings from different authors to consolidate the results from the literature study. Misinterpretation or misunderstanding might also influence the outcome.
%\end{itemize}
\end{comment}




\begin{comment}
Regarding the retrieves quadrant, a surprising benefit of \copilot{}s is their ability to retrieve and reframe formal methods, as suggested by Ferrari and Spoletini \cite{10.1016/j.infsof.2025.107697}.
They argue that by bridging natural and formal language, \copilot{}s can make formal specifications accessible to practitioners, thereby retrieving rigor and guarantees that were previously reserved for experts.


Similarly, the revival of test-driven development (TDD) as a strategic paradigm shift is retrieved through copilot support (Sauvola et al. \cite{10.1007/s10515-024-00426-z}), reinforcing the value of executable specifications.

Prioritization of rapid prototyping by Rico and Öberg \cite{10.1145/3696630.3728718} and Terragni et al. \cite{10.1145/3715003} also signals a return to earlier ideals of flexibility and exploratory design phases that predate heavy plan-driven methodologies.

To summarize, generative AI tools in software engineering reintroduce and amplify concepts that had become less central in modern workflows.
A prominent example is the renewed interest in \textit{Formal Verification and Specifications}.
Once considered the domain of highly specialized contexts, formal methods are now made more accessible through natural language interfaces, enabling wider adoption and integration into early development stages (Ferrari and Spoletini~\cite{10.1016/j.infsof.2025.107697}).
Complementarily, the use of \textit{Natural Language as a Specification Medium} has become increasingly viable, as developers can articulate complex intentions through expressive prompts that guide code synthesis (Kam et al.~\cite{10.1145/3696630.3727251}).
This shift helps bridge the gap between business stakeholders and technical teams.
Moreover, the rapid feedback loops enabled by AI tools revive the centrality of \textit{Prototyping and Iterative Design}, reinforcing exploratory development and experimental cycles that mirror agile and Lean principles (Sauvola et al.~\cite{10.1007/s10515-024-00426-z}; Qiu et al.~\cite{10.1145/3709353}).
Another classic methodology that resurfaces in this AI-driven landscape is \textit{Test-Driven Development (TDD)}; aided by AI companions capable of generating and refining test cases, TDD evolves into a more integrated and less burdensome practice (Wang et al.~\cite{WangHCLWW24}).
Finally, these developments contribute to a broader retrieval of \textit{Developer Creativity} as a key asset: tools such as \copilot{} not only automate implementation but also act as thought partners, assisting with brainstorming and expanding the solution space (Terragni et al.~\cite{10.1145/3715003}).
Together, these retrieved practices suggest that while AI represents the future of software engineering, it simultaneously reconnects the field with enduring principles and methods that remain foundational.
\end{comment}




% \andreas{potentially relevant papers: \url{https://abhikrc.com/pdf/Agent.pdf}; \url{https://arxiv.org/abs/2410.06107}}

% \tobias{During our search we found the following papers that might be interesting for the Agent-case:}
% \begin{comment}
% -SimAC: Simulating Agile Collaboration to Generate Acceptance Criteria in User Story Elaboration; https://doi.org/10.1007/s10515-024-00448-7
% -Self-Collaboration Code Generation via ChatGPT; https://doi.org/10.1145/3672459
% -SpecRover: Code Intent Extraction via Llms; https://doi.org/10.1109/ICSE55347.2025.00080
% -Software Engineering Using Autonomous Agents: Are We There Yet?; https://doi.org/10.1109/ASE56229.2023.00174
% -UI2HTML: Utilizing LLM Agents with Chain of Thought to Convert UI into HTML Code; https://doi.org/10.1007/s10515-025-00509-5
% -Enhancing Human-IDE Interaction in the SDLC Using LLM-based Mediator Agents; https://doi.org/10.1145/3696630.3728721
% -Mediating between Human Programmers and Integrated Development Environments Using LLM-based Agents; https://doi.org/10.1145/3696630.3731460
% Empowering Agile-Based Generative Software Development through Human-AI Teamwork; https://doi.org/10.1145/3702987
% LLM-based Multi-Agent Systems for Software Engineering: Literature Review, Vision, and the Road Ahead; https://doi.org/10.1145/3712003
% \end{comment}

\begin{comment}
\subsection{Validity Risks}
\label{sec:validity2}

This Rapid Literature Review presents some validity threats by its design. Since systematicity was not the focus of this study, subsequent iterations of the research approach may lead to slightly different results.
Additionally, the applied search string was designed to be strict; therefore, we may have missed some relevant literature items. The search was conducted in the main Scientific Database aggregators (Scopus and Google Scholar) and the main Software Engineering conferences, though some relevant literature items may have been only indexed in other AI or Machine Learning-centered conferences.

% \andreas{Quite recent google release:} \url{https://android-developers.googleblog.com/2025/06/agentic-ai-takes-gemini-in-android-studio-to-next-level.html?utm_source=email&utm_medium=newsletter&utm_campaign=dev_program_july}
\end{comment}


\begin{comment}
    

\subsection{Validity Risks}
\label{sec:validity3}

Given the large number of publications retrieved by the search, we applied a first filter using Qwen3, looking at paper title, abstract, and keywords.
As a result of this decision, papers not mentioning explicitly topics relevant to \aiware{} in title, abstract and keywords may have been discarded.
Moreover, due to the chance of the LLM making mistakes, there may have been papers wrongfully discarded.
\end{comment}

\begin{comment}

\andreas{Braindump Andreas:}
\begin{itemize}
    \item \textbf{Promptware / AI-WARE / DevOps 2.0}
    \begin{itemize}
        \item IdeaAM: novel programming language that combines programmatic structured programming with prompt-based texting.
        \item Current prompt development practices are often ad hoc and experimental, relying on trial-and-error $\rightarrow$ "promptware crisis".
        \item Lack of systematic approaches for prompt engineering.
        \item As LLMs become crucial in software engineering workflows, current ad hoc prompt development methods are unsustainable.
        \item Unlike conventional software, promptware uses natural language as its "code".
        \begin{itemize}
            \item Natural language is flexible, context-dependent, ambiguous, complicating prompt construction and analysis.
            \item Promptware operates on probabilistic, non-deterministic LLM runtime environments.
            \item $\rightarrow$ Unique complexities: human-like behaviors, unclear capabilities, undefined error handling, uncertain execution outcomes complicate reliable software development.
        \end{itemize}
        \item Paradigm shift to probabilistic, natural language prompts alters definition of "software" and "software development".
        \item $\rightarrow$ Apply rigorous Software Engineering principles to prompt development.
        \item Promptware Engineering: Software Engineering for LLM Prompt Development; \url{https://arxiv.org/abs/2503.02400}
    \end{itemize}
\end{itemize}

\tobias{"An Exploratory Study of V-Model in Building ML-Enabled Software: A Systems Engineering Perspective" \url{https://doi.org/10.1145/3644815.3644951}}

NOTE: Here is a very simple example for the impact of AIWARE on the lifecycle, i.e., in addition to the SDLC, we will need an alignment and integration with the prompt and data lifecycles:

\includegraphics[width=.4\textwidth]{imgs/aiware-lc.png}
\end{comment}


\begin{comment}
    \subsection{3rd Cycle -- Final Artifact Development}
\label{sec:cycle3}
The third cycle was mostly dedicated to the final artifact development and validation. %dedicated to consolidation, refinement, and validation.

\subsubsection{Awareness - Consolidation}
First, McLuhan's tetrads were updated by the individual author teams based on feedback from internal peer review.
\pat{describe better}


\subsubsection{Solution - Updated McLuhan's Tetrads of \ai in SE}
Then, the WHO? jointly identified similar or common elements across the Tetrads for the four different forms of \ai in SE, leading to a set of overall research challenges and opportunities.
\pat{describe better}

\subsubsection{Validation - Cross Validation}
Finally, these findings were cross-validated by WHO?.
This final cycle thereby ensured consistency and robustness, leading to a set of validated research challenges and opportunities.
\pat{describe better}

\marco{Yes, I also agree, the above should be clarified a bit}
\end{comment}


\begin{comment}
    


\begin{enumerate}[label=\textbf{E\arabic*.}, leftmargin=*]
\item \textbf{Hybrid systems: integrating process agents + product agents}

\textit{Challenge}: In future systems, process-level agents (that plan development) and product-level agents (in software) may co-exist and influence each other. Managing their interactions is complex. \\
\textit{Opportunity}: Architectures and protocols for cross-layer consistency, feedback loops, negotiation, and coordinated evolution.

\item \textbf{Metrics, evaluation benchmarks, and empirical validation}

\textit{Challenge}: How do we measure ``goodness'' of GenAI augmentation (for productivity, reliability, maintainability, human satisfaction)? \\
\textit{Opportunity}: Define standard benchmarks, controlled experiments, and evaluation suites for hybrid human-AI engineering settings.

\item \textbf{Human factors, team dynamics, education and roles}

\textit{Challenge}: As GenAI changes workflows, roles and skills shift. Resistance, cognitive burden, misuse, or misalignment may arise. \\
\textit{Opportunity}: Study human-AI teaming, change management, training curricula, and social/organizational adaptation strategies.

\item \textbf{Intellectual property, licensing, and legal liability}

\textit{Challenge}: Who owns code, designs, or artifacts generated by GenAI? What licenses apply? What liability when AI-generated code fails? \\
\textit{Opportunity}: Legal and policy frameworks for IP attribution, shared licensing models, AI-generated artifact contracts, and compliance regimes.

\item \textbf{Energy, sustainability, and carbon cost}

\textit{Challenge}: Running large models (during development or deployment) has nontrivial environmental cost. \\
\textit{Opportunity}: Energy-efficient model architectures, selective inference, energy-aware scheduling, and carbon‑aware software engineering.

\item \textbf{Model robustness, adversarial attacks, and misuse}

\textit{Challenge}: GenAI elements and agents can be manipulated via adversarial prompts or injection attacks to produce harmful outputs. \\
\textit{Opportunity}: Robustness research, prompt sanitization, query filtering, anomaly detection, and secure input/output boundaries.

\item \textbf{Domain-specific adaptation and transferability}

\textit{Challenge}: Models and augmentation methods developed in one domain (e.g., web apps) may not transfer to, say, embedded systems, safety-critical domains, or regulatory contexts. \\
\textit{Opportunity}: Techniques for domain adaptation, modularization, few-shot tuning, and adaptation frameworks for engineering domains.

\item \textbf{Sustainability of knowledge, evolving software landscapes}

\textit{Challenge}: The software ecosystem (languages, frameworks, libraries) evolves rapidly; GenAI augmentation must keep up. \\
\textit{Opportunity}: Continual learning, modular plugin adaptation, community-based model updates, and open model ecosystems in the software engineering domain.
\end{enumerate}

\end{comment}



\subsection{(Current) Limitations and Impacts of \ai{} for SE \pat{here focus on \ai{} for SE and the previous section \ai{} in SE? Why in this case we only focus on limitations and impacts? }}
\label{sec:limitations}



\noindent\textbf{Reproducibility:}
A fundamental challenge with \ai{} is its inherent lack of reproducibility or replicability~\cite{baltes2025,zhou2023}.
Due to the "random noise" integral to their operation, \ai{} models rarely produce the exact same output, even when given the same prompt.
This variability can be a significant obstacle in software engineering, where consistency and predictability are often paramount.
%
\marco{Check if more clear now} \ins{While model configuration parameters like "temperature" (which controls how creative or precise the model is) and "top\_p" (nucleus sampling, which limits the model's choices) can be set to zero to reduce non-determinism to some extent, they do not entirely eliminate the issue.}
%
The inability to guarantee identical results for the same input poses a challenge for SE, e.g., for standardized testing and validation processes.

\noindent\textbf{Bias:}
\ai{} models can perpetuate and even amplify biases present in their training data~\cite{baltes2025}.
One classical example is prompting an LLM to generate images of "watches showing 12:00", which typically produces a set of watches showing 10:10 (the most proliferating way of how watches are photographed), reflecting a lack of diversity in its training examples.
Such biases can lead to inaccurate or unfair outcomes.
For example, this could manifest itself as biased test case generation, where \ai{} focuses on common scenarios and neglects edge cases.

\noindent\textbf{"Clever Hans" Effect:}
\ai{} models may learn from irrelevant or spurious features in the training data, a phenomenon known as the "Clever Hans Effect"~\cite{Kauffmann25}.
This is named after a horse that appeared to perform intellectual tasks, but was actually reacting to subtle, involuntary cues from its trainer.
In the context of \ai{}, this means that the \ai{} model may not be learning the underlying principles but is instead relying on superficial correlations.
In SE, this could lead to a \ai{} model that appears to correctly identify bugs but is actually relying on irrelevant code formatting or comments, making it unreliable when faced with new, differently styled code.

\noindent\textbf{Data Pollution:}
The integrity of benchmark datasets used to evaluate and compare \ai{} solutions may be compromised through `Data Pollution' (aka. `Data Contamination' or `Benchmark Contamination')~\cite{baltes2025,zhou2023}.
This occurs when a \ai{} model has been accidentally or intentionally exposed to the benchmark data during its training or fine-tuning phase.
This has several negative consequences:
\begin{itemize}
    \item \textit{Artificial Overestimation -} The \ai{} model's performance will be artificially inflated, giving a false sense of its capabilities;
    \item \textit{Compromised Evaluation Integrity -} The purpose of a benchmark is to objectively measure performance on unseen data.
    Contamination undermines this, making it difficult to reliably compare different AI techniques;
    \item \textit{Poor Real-World Performance -} A \ai{} model that excels on a contaminated benchmark is likely to perform poorly in real-world applications where it encounters truly novel data.
\end{itemize}

\noindent\textbf{Resource Usage and Sustainability:}
While the energy efficiency of \ai{} hardware improves significantly each year, the size and complexity of \ai{} models are growing at an even faster rate.
This rapid growth in model size together with the increased deployment and usage of these models often cancels out the hardware efficiency gains.
This situation is an instantiation of the "Jevons paradox", where increased efficiency in resource use leads to a higher overall consumption of that resource.
In the case of \ai{}, as the technology becomes more efficient and less costly, its adoption and usage increase, leading to a greater total energy consumption and negating the initial efficiency improvements.
Increasing the level of \ai{} augmentation of software systems (in the form of \aiware and \robot{}s) thus may lead to a significant increase in resource usage of future software systems and thus may present a sustainability challenge if such AI-augmented systems are widely deployed and used.

% \textbf{Technical Debt:}
%% // I removed this, as in the end GenAI will rather help address tech debt -- via refactoring; at least I could not find a decent paper that supports this "negative" view wrt tech debt
% The ease with which \ai{} can generate code (and other SE artifacts) can lead to an accumulation of technical debt [cite: 15].
% Developers may be tempted to quickly generate and duplicate code rather than engaging in more effortful but sustainable practices like refactoring [cite: 15].
% This leads to a "Don't Repeat Yourself" (DRY) principle being replaced by constant duplication.
% % [cite_start]The bar chart showing the "Percent of Changed Lines Moved for Refactoring, by Year" from 2021 to 2024 indicates a declining trend in refactoring, suggesting that developers are increasingly opting to add new, AI-generated code instead of improving existing code[cite: 15].
% As a result development repositories and code-bases will become difficult to maintain and evolve over time.

\noindent\textbf{Team Dynamics and Skills:}
Integration of \ai{} into SE is poised to significantly change team dynamics.
Senior team members may transition into supervisory roles, managing \teammate{}s (realized as \ai{} agents), while junior members will need to engage in continuous and accelerated learning to stay up to date.
Empirical data from a Harvard Business School study shows that both individuals and teams see a notable improvement in the quality of their work when using \ai{}~\cite{dell2025}.
However, to effectively leverage \ai{}, there is a growing need for skilled personnel who can develop, implement, and maintain these AI-augmented tools and systems.
Organizations will need to invest in training and development to equip their SE teams with the necessary \ai{} skills, a requirement that is also mandated by legislation such as the European Union's AI Act\footnote{\url{https://digital-strategy.ec.europa.eu/en/policies/regulatory-framework-ai}}.

\begin{comment}

% \pat{this paper of Mauro can be used as motivation~\cite{TOSEMPezze2025}, Section 2 Software Development in the Era of AI:
% {\em To keep pace with such complexity, developers innovate and adopt new processes, novel technologies, and powerful automation to augment their capabilities for creating and orchestrating how software system versions are managed by these distributed networks of thousands of developers. These innovations, such as the Internet and social coding tools, and processes, such as agile, change not just the speed and quality of the software being developed, but they also alter the very essence of how software is authored by developers, and the ways they work together.}}

% \pat{Check also this: 3.3 From NoOps to AIOps~\cite{TOSEMPezze2025}, and the highlighted open Challenges: Section 3.3.2 Open Challenges, and Section 3.3.3 Roadmap}

% \pat{Check also this from~\cite{TOSEMPezze2025}:
% (3)
% What future SE processes will we see in 2030 and beyond?
% AI dramatically redefines the SE process:
% (3.1)
% Psychological operations in SE. How will we support psychological operations and manage AI fatigue in SE? (see Section 3.3)
% (3.2)
% Orchestration. How will we merge explainable AI approaches with cloud and edge principles into explainable meta-orchestration with human layers? (see Section 3.3)
% (3.3)
% Superconnectedness. How will we measure and manage superconnectedness and disconnectedness in data meshes? (see Section 3.3)}

% The remainder of this article is structured as follows.
% EXPLAIN


    
\tobias{Discuss agentic vs. gen AI }

I analyzed some papers from last year's special issue and observed that:

\begin{itemize}
    \item \textbf{First observation:} Many papers in the section ``Artificial Intelligence for Software Engineering'' discuss the use of LLMs or generative AI in software engineering.
    \item \textbf{Second observation:} Perhaps only one of these papers uses a systematic approach and reports a well-defined process.
    \item \textbf{Third observation:} Almost all of these papers present a state of the art, even if it was not done systematically. They then proceed to discuss future visions and research directions.
    \item \textbf{Fourth observation:} By reading the other sections, such as ``Software Engineering by and for Humans,'' I noticed that the practice is similar. Almost all papers first provide an overview of the current state, sometimes using systematic approaches such as literature reviews, mappings, etc., and then move on to challenges, research directions, and visions.
\end{itemize}


possible directions:


\begin{enumerate}
    \item Be formal and provide evidence for everything, using a combination of rapid literature review and grey literature review (e.g., blogs, YouTube videos, etc.) to give an overview of the current state of the use of GenAI in development processes. We could also use interviews to:
    \begin{itemize}
        \item validate the state of the art (as Andreas did in the interviews),
        \item provide evidence, or at least a broader perspective, regarding future research directions and/or visions. 
    \end{itemize}
    Of course, this process, which I tried to outline in the design science approach in figure \ref{fig:designscience}, requires more time.

    \item Remove the methodology, not having a guiding process, but instead describe the state of the art, future research directions, and/or visions from our point of view, offering a limited perspective by design, regarding the use of GenAI in development processes.
    

    \item A mix? For instance, we could conduct a state of the art ourselves (like related work, without using a systematic study) and use the interviews only to validate the state of the art, as well as to get a point of view on future research directions and/or visions on the use of GenAI in development processes.

    \tobias{With the last two we could take our workshop proposal as one case that is discussed in more detail, instead of being vague with everything. Maybe we then need a second case to not seem too focussed}
    \item Other suggestions?
\end{enumerate}
\end{comment}


==> copilot_detailed.tex <==
\section{Impact of \copilot{}s on the Life-cycle}
\label{sec:copilot}

As introduced in Section~\ref{sec:taxonomy}, a \copilot{} is a component or service that supports human software engineers in carrying out development tasks.

% \andreas{some papers I found: \url{https://www.sciencedirect.com/science/article/pii/S0950584925000904}; \url{https://dl.acm.org/doi/abs/10.1145/3696630.3730538}}

\subsection{Rapid Literature Review}
\label{sec:review1}

To provide an overview of the implications and impacts of \copilot{}s on the \sdlc, as already addressed in the literature, we performed a rapid literature review.

\subsubsection{Review Approach}
\label{sec:review_approach1}
The overall procedure we followed to perform the rapid literature review for \copilot{}s is depicted in \autoref{fig:copilot-review}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth, trim=0cm 1cm 0cm 1.2cm, clip=true]{imgs/rr_process_copilot.pdf}
    \caption{Identifying relevant publications concerning \copilot{}s \pat{let's try to follow a uniform protocol in the four parts. The search string of Section 5 is using ABS here not... OR we should be more clear on what a rapid literature review is, why here we don't use scopus later we do, etc.}}
    \label{fig:copilot-review}
\end{figure}

As this category of \ai has attracted the most research focus in software engineering to date, we limited our search to top-tier software engineering conferences and journals (ICSE, ASE, FSE, TOSEM, TSE, EMSE, JSS, IST, ASEJ).
We restricted the search to the years 2019--present, as the first Transformer-based models (BERT and GPT) were released in 2018, requiring time for adoption by the SE community.
To ensure comprehensive coverage, we opted for full-text searches using ACM and IEEE as search engines, as we initially found that many papers only discuss the impact on the \sdlc in the body of the paper and not the title, abstract, or keywords.
We narrowed the scope to papers explicitly mentioning the \sdlc, development process, or software engineering process in conjunction with LLMs, \ai, or transformer architecture.
These criteria are reflected in the search string presented in \autoref{fig:copilot-review}.

To further streamline the analysis process, we leveraged \marco{Maybe we better add a link to Qwen3 in a footnote?} Qwen3 to analyze the titles, abstracts, and keywords of retrieved publications.
%We asked the model to separately address two questions about each publication:
We asked the model to answer two questions about the publication that reflect the scope of our search:
(Q1) Whether the paper explicitly discusses the role and/or implications of \ai on the \sdlc;
(Q2) Whether the paper utilizes \ai or LLMs as a tool to support or automate tasks along the \sdlc (not as integral components of the software system, product, or application).
Q1 focuses on the publication's scope, while Q2 excludes \aiware or \robot publications, focused on in the following chapters.
For each question, Qwen3 provided a yes/no answer along with its reasoning\footnote{Results are available in our replication package (TODO)}.
Publications positively evaluated by Qwen3 for both questions were then manually inspected by two authors (split equally).





%Use full text search on ACM and IEEE for top-tier SE conferences and journals: ICSE, ASE, FSE, TOSEM, TSE, EMSE, JSS, IST\\
%time frame: 2019-today
%Full text more helpful than title-abs because most papers only talk about impact in the body\\


%Results: 385 unique papers

\subsubsection{Review Results}
\label{sec:review_results1}
The initial search in ACM and IEEE resulted in 385 publications.
Qwen3 classified 161 of these as discussing the role or implications of \ai on the \sdlc and 191 as utilizing \ai as a tool to support or automate tasks along the \sdlc.
147 of these fulfilled both criteria and were manually inspected.
During the manual inspection process, the authors identified that most publications only mention the \sdlc as motivation or in the related work, but do not describe the implications of \ai on it (100 papers).
Additionally, many publications made only single statements about the impact or role of \ai in the \sdlc, or single tasks of the \sdlc that are improved (32 papers).
Only a few publications provided a broader discussion of the implications and role of \copilot{}s on the \sdlc (15 papers, see Table \ref{tab:copilot-sota}).

The latter two categories were used to inform our McLuhan's tetrad (see \autoref{sec:roadmap1}), either by deriving insights from the single statements or analyzing the full discussion in the 15 other papers.
Additionally, we included our proposal for the Future Software Engineering Workshop @FSE2025 (FSEws2025) on \enquote{Automated Knowledge Management in the Software Life Cycle} \cite{keim_automated_2025}, as it was one of the starting points for this contribution and fits into the \copilot category.

From the "Single Statement or Tasks" publications we derived the following initial statements categorized along McLuhan's tetrad dimensions: \pat{this are kind of working details. We can move this to the replication package.}
\begin{enumerate}[wide=0pt, labelindent=0pt, align=left]
    \item[\textbf{Enhances:}]  \textit{Vulnerability Detection},
    \textit{Assurance Case Generation},
    \textit{Identifying relevant documents for SE tasks (Code discovery, Traceability, ...)},
    \textit{Understanding of software projects}, % Make design rationales from open-source communities available,
    \textit{Onboarding},
    \textit{Validation and Testing}, % unit, usability, prototyping ...
    \textit{Bug fixing},
    \textit{Code comprehension},
    \textit{Automated Debugging},
    \textit{Code Refinement},
    \textit{Test design},
    \textit{Coding (literate, faster)},
    \textit{Feedback to developers (Continuous, real-time)}, % on vulnerabilioties, bug fixes, tests
    \textit{Quality assurance (continuous)},
    \textit{Detection of incompleteness, inconsistencies and discrepancies throughout the life-cycle}.
    \item[\textbf{Reverses:}] \textit{Trustworthiness of SE tools},
    \textit{Fairness of SE tools},
    \textit{Compliance with all requirements and policies}.
    \item[\textbf{Retrieves:}]\textit{Rapid release cycles},
    \textit{TDD}, % LLMs embrace TTD as strategic paradigm shift
    \textit{Creative insights and ideas for developers}.
    \item[\textbf{Obsolesces:}] \textit{Manual portation to other languages},
    \textit{step-by-step program repair}, %enable end2end program repair
    \textit{manually defining development workflows}, % write dev workflows as software
    \textit{traditional verification and validation processes}, %highly advanced morescient models to accurately predict the execution of software, making traditional verification and validation processes largely obsolete or redundant
    \textit{Eliciting requirements from memorized stakeholder conversation}, %Automatically generate requirements candidates from stakeholder conversations
    \textit{Transferring sketches to code}.
\end{enumerate}


%The relevant publications concerning \ai{}-Co-Pilots that include a broader discussion of the impact on the SDLC than simple statements of \ai improves a certain SE task are listed in Table~\ref{tab:copilot-sota}.

\begin{table}[]
    \centering
      \caption{Relevant publications concerning \copilot{}s}
   \label{tab:copilot-sota}
   \rowcolors{2}{white}{gray!25} % every 2nd row shaded
    \footnotesize
    \begin{tabularx}{\textwidth}{Xlc}

    \toprule
    Paper & Authors & Year\\
    \midrule
    Future of software development with generative AI \cite{10.1007/s10515-024-00426-z} & Sauvola et al. & 2024\\
A disruptive research playbook for studying disruptive innovations \cite{10.1145/3678172} & Storey et al. & 2024\\
Large language models for software engineering: a systematic literature review \cite{10.1145/3695988} & Hou et al. & 2024\\
Software testing with large language models: Survey, landscape, and vision \cite{WangHCLWW24} & Wang et al. & 2024\\
Formal requirements engineering and large language models: A two-way roadmap \cite{10.1016/j.infsof.2025.107697} & Ferrari and Spoletini & 2025\\
Copiloting the future: How generative AI transforms software engineering \cite{10.1016/j.infsof.2025.107751} & Banh et al. &2025\\
Challenges and opportunities for generative AI in software engineering: a managerial view \cite{10.1145/3696630.3728718} & Rico and Öberg &2025\\
What do professional software developers need to know to succeed in an age of Artificial Intelligence? \cite{10.1145/3696630.3727251} & Kam et al.&2025\\
AI in the software development lifecycle: Insights and open research questions \cite{10.1145/3696630.3730538} & Guimaraes and Nascimento &2025\\
The future of AI-driven software engineering \cite{10.1145/3715003} & Terragni et al. &2025\\
From today's code to tomorrow's symphony: The AI transformation of developer's routine by 2030 \cite{10.1145/3709353} & Qiu et al. &2025\\
From triumph to uncertainty: The journey of software engineering in the AI era \cite{10.1145/3709360} & Mastropaolo et al. &2025\\
Automatic programming: Large language models and beyond \cite{10.1145/3708519} & Lyu et al. &2025\\
The current challenges of software engineering in the era of large language models \cite{10.1145/3712005} & Gao et al.&2025\\
Artificial intelligence for software engineering: The journey so far and the road ahead \cite{10.1145/3719006} & Ahmed et al.&2025\\
Towards Automated Knowledge Management in the Software Life Cycle \cite{keim_automated_2025} & Keim et al.&2025\\
    \bottomrule
    \end{tabularx}

   % }
\end{table}
Sauvola et al. \cite{10.1007/s10515-024-00426-z} mention that \ai will make strict boundaries between \sdlc stages disappear % (design, coding, testing, and deployment may overlap, or disappear)
and rapid prototyping will become more reasonable again.
They structure their analysis according to four potential adoption scenarios: Traditional Software Development Operations, AI in the loop, AI assumes role(s), and Human-in-the-loop.
The first two correspond to our \copilot category and the authors mention in their analysis enhancements of code comprehension, code generation, debugging, testing, deployment, and maintenance as well as automating repetitive and even customer (DevOps) facing tasks. For simpler applications, they envision zero- and no-code environments, or code generation services.

Storey et al. \cite{10.1145/3678172} provided a McLuhan's tetrad for code generation, from which we derived that documentation, productivity and quality are \textit{enhanced}, individual understanding capabilities of developers are \textit{reversed}, natural language explanation of code are \textit{retrieved}, and the need for search of code snippets and the need for manually created documentation are made \textit{obsolete}.

In their systematic literature review from 2024, Hou et al.~\cite{10.1145/3695988} present the key applications of LLMs across the \sdlc stages and summarize the key challenges of using them in software engineering.
They found that the majority of publications using LLMs are targeting tasks in the software development stage (57\%), followed by software maintenance (23\%) and quality assurance tasks (15\%).
Applications in requirements engineering, software design, and management were targeted by less than 5\% of studies.
As challenges, they identified LLM applicability challenges, such as model size and deployment, data dependency, or ambiguity, the challenge of generalizability, challenges in evaluating LLMs, and the interpretability, trustworthiness, and ethical usage of LLMs in SE.
As a roadmap for future developments, they see enhancements in automated coding, development, personalized developer assistance, testing and analysis, code reviews and quality assurance, predictive analysis and decision support, as well as software security.

Wang et al.~\cite{WangHCLWW24} performed a similar study but narrowed the scope to software testing.
They discovered that LLMs are primarily used to enhance tasks in the middle to later stages of the software testing life cycle (functional/unit/system tests), whereas early stages and non-functional testing are underexplored.
In general, they report that LLMs can enhance test case generation, bug detection, and program repair and debugging, leading to faster testing cycles and enhanced coverage.
By this, tasks such as manual writing of tests, oracles and test inputs, as well as hand-debugging and manual bug reproduction become less central.
However, they also report some challenges or risks, such as shallow coverage of generated tests, weak test oracles, and reliability.

Ferrari and Spoletini \cite{10.1016/j.infsof.2025.107697} present a two-way roadmap for using LLMs in requirements engineering.
They envision that formal methods are used to provide guarantees for outcomes produced by LLMs and, at the same time, LLMs can make formal methods more accessible.
LLMs can enhance the extraction, analysis, verification, and validation of requirements.
By bridging the gap between natural language and formal specifications, it can retrieve the rigor and guarantees formal methods provide for practitioners not familiar with formal methods.
This could reduce the need for manual requirements elicitation and specialized formal methods experts for routine tasks.
However, blindly trusting the LLMs could also lead to superficial applications of formal methods without deeper foundations, both theoretical and context-wise.

Banh et al. \cite{10.1016/j.infsof.2025.107751} conducted expert interviews with 18 professionals and grounded theory to analyze both the opportunities and challenges associated with \ai adoption in software development workflows.
They describe that the advanced reasoning capabilities of \copilot{}s enable code analysis, conceptualization, and natural language coding.
Furthermore, by enhancing developer productivity through, e.g., code refinement, error identification, and providing contextual knowledge, the code quality and development time can be improved.
However, they also discuss the issues of reliability and intellectual property and the resulting, often underestimated overhead.

Rico and Öberg \cite{10.1145/3696630.3728718} gather insights from a workshop with eight managers and team leaders from diverse organizations on the actual uses of LLMs and practical challenges.
The managers acknowledged that LLMs could generate and refine requirements or produce automated design protocols and could enhance the time required, especially in situations where documentation is voluminous.
They also see automated debugging and real-time code analysis and optimization as "game-changers".
For testing and quality assurance, the managers believe that quality assurance workloads could be reduced and more defects could be caught early, by automating test generation and synthetic data creation.
Additionally, the managers saw potential for AI-driven effort estimation, coaching and training opportunities.
As challenges, they described reliability and trustworthiness issues, intellectual property concerns, and concerns of lower quality and higher security risks of \ai{}-generated code.

Kam et al. \cite{10.1145/3696630.3727251} surveyed developers to discover insights on how AI is reshaping the work of developers.
To come to these insights, the authors first assess the current usage of AI for development.
This usage includes, among others, finding the location of information, exploring solutions, generating code, assets, or documentation, and performing code analyses to improve code quality.
The authors map the 75 AI-enabled developer tasks to each stage of the \sdlc.
Based on this, the authors come to various insights.
For example, AI will enhance the process as it will be used to optimize for both business metrics and engineering metrics.
Further, AI-driven development will enhance efficiency.
Moreover, AI will likely lead to enhanced communication as less time is wasted answering easy questions and more time can be used for meaningful questions.
The authors state that the changes from AI will require a slightly different, nuanced set of skills.
When interacting with AI, developers will follow a six-step task workflow with the steps \textit{identify}, \textit{engage}, \textit{evaluate}, \textit{calibrate}, \textit{tweak}, \textit{finalize}.

Guimaraes and Nascimento \cite{10.1145/3696630.3730538} examine AI's evolving role in code generation, testing, debugging, software architecture, and maintenance.
To do so, they form a phase-wise perspective.
For each phase, the authors identify multiple opportunities to enhance the current process and to make it more efficient, with most of these enhancements stemming from automation.
However, the authors also identify challenges related to reliability, robustness, trustworthiness, security, explainability, transparency, legal, and ethical concerns.
Furthermore, the authors see challenges in fostering Human-AI collaboration, such that efficiency and seamless developer collaboration can be emphasized.

Terragni et al. \cite{10.1145/3715003} present their vision of the potential future of an AI-driven software engineering, based on a current snapshot of (AI) tools in software development.
In this future, the authors see AI as the main actor besides the developers, and developers can either directly operate on artifacts or use AI.
As such, communication between the developers and AI will be essential.
Similar to other work, Terragni et al. see AI as a supporting tool to enhance the \sdlc.
Examples for the use of AI are rapid prototyping, stakeholder-specific documentation, code quality, and updates, among others.
However, they also see potential that certain parts of requirements elicitation can become obsolete, like the involvement of requirements engineers for elicitation.
\marco{Sentence to be checked} The authors again see Explainable AI and testing as crucial aspects as well as ensuring that the artifacts are compliant to relevant licenses.

Qiu et al. create projections for 2030 and focus, in particular, on the implementation as \enquote{pivotal phase} \cite{10.1145/3709353}.
In their projection, an AI-assistant can enhance development with five tools: mental health monitor, fault detector, code optimizer, team coordinator, and skills advisor.
In addition to things also mentioned by other scientists, the authors include factors that directly improve the developer's health by enabling better focus or adapting the environment (e.g., color schemes, font sizes).
Further, the authors see that AI-assistants can lead to smart teams that have improved interaction with more useful meetings, leading also to enhanced task distribution.
Lastly, AI-assistants might detect required skills and enhance how developers learn these skills in tailored learning paths.

Mastropaolo et al. \cite{10.1145/3709360} discuss the history and impact of AI on the \sdlc, focusing on concerns and questions that will likely arise.
Apart from the previously mentioned concerns, the authors add additional ones, looking at different angles and problem areas, including the training and benchmarking of LLMs for coding.
The authors also view the enhancements of AI as a double-edged sword, given the threats to trust, accountability, legal compliance, as well as algorithmic bias, energy efficiency and sustainability, and security.
In the SE of the future, the view on software engineers and their roles can change drastically, and a wide number of concerns will arise.
Among others, they ask whether humans or AI should produce code, which parts should either one produce, or if AI should have project management capabilities.

Lyu et al. \cite{10.1145/3708519} examine how trust boundaries can shift when we integrate automatically generated artifacts into a software project.
As such, they focus on the concerns and remedies.
When integrating generated code, the authors identify concerns regarding security, reliability, and privacy.
Additionally, the authors look into the interaction between developers and AI and also identify two common patterns: \textit{autocompletion} and \textit{prompting}.
In the \sdlc and, in particular, maintenance and evolution, the authors see enhancements in summarization of code and code changes, but also in automated code reviews.
They envision different roles for the programmer, like being a code designer instead of a code writer or being a quality assurance specialist.

Gao et al. \cite{10.1145/3712005} look into the current challenges of LLMs for software engineering along the \sdlc and the implications for the future.
As such, the authors look into requirements and design, coding assistance, test code generation, code review, software maintenance, and vulnerability management, as well as data, training, and evaluation.
In all these phases, AI assistants are used, posing corresponding challenges, with an overarching challenge of building LLMs and AI assistants.
According to the authors, we first need to understand these challenges and solving them might result in changes and enhancements of the current process.

Similarly, Ahmed et al. \cite{10.1145/3719006} identify the open technical and organizational challenges and construct a roadmap that outlines the envisioned 2030 research horizon.
In this roadmap, the authors see, among others, enhancements regarding robust safeguards to ensure fairness, transparency, and accountability.
The \sdlc will be further enhanced through optimizations and improvements of current processes.
The supply chain of software construction, delivery, and maintenance will be important in this change.
Further, AI will take over repetitive tasks and can help improve code and product quality.
However, adverse effects like overreliance on AI, job displacement due to outsourcing tasks to AI, and bias that can lead to unfair or discriminatory results might affect the future software engineering discipline and the \sdlc.

Keim et al. \cite{keim_automated_2025} envision holistic knowledge management across the entire life cycle.
They want to exploit LLMs in conjunction with data coming from all artifacts to automatically manage knowledge and check the consistency of artifacts against such knowledge.
This envisioned approach will be able to process each artifact to extract knowledge, check the consistency with existing knowledge, and update the knowledge base.
If inconsistencies are found, LLMs can help explain the inconsistencies and the user can act accordingly.
The knowledge can also enhance human-computer interaction, contextual learning and processing, and working in new domains.
The authors also mention challenges similar to previously enumerated challenges, like explainability, trust, or defect prediction.
\marco{Not a clear sentence to be polished} These challenges can come up with such an approach but where the approach can also partly help, for example, with showing the source of certain knowledge or with explanations about the inconsistencies.


\subsection{Roadmap (McLuhan's tetrad)}
\label{sec:roadmap1}
\input{figures/mcluhans_tetrad_copilot}
Mapping and consolidating the different impacts and implications of \copilot{}s on the \sdlc discussed in the literature resulted in the McLuhan's tetrad shown in \autoref{fig:tetrad-copilots}.
Most work focuses on enhancements of current processes and activities, where GenAI copilots will enhance nearly every stage of software engineering by assisting with requirements elicitation, design, coding, debugging, testing, documentation, team collaboration, and developer productivity.
However, they will also retrieve older practices and ideals such as formal specifications, formal verification, test-driven development, rapid prototyping, and providing creative insights and natural language explanations.
At the same time, they will make several traditional practices obsolete, such as manual debugging, manual test creation, hand-written documentation, requirements elicitation, and manual porting between languages. However, they also reverse and raise concerns around trust, fairness, individual understanding, sustainability, and the loss of strict boundaries and ownership within the SDLC.

\begin{comment}
    A discussion with participants of the Requirements Engineering conference 2025 (RE2025) also resulted in the following ideas\pat{didn't find this on the research methodology. It comes out of the blue.}:
\begin{itemize}
    \item Requirements engineering gets more important than ever, if they are regarded as the input on which the following steps are (semi-) automatically performed.
    \item There can be the ability to scale requirements elicitation to many stakeholders, without additional costs, by performing the interviews with LLMs.
    \item There might be the possibility to check the consistency of requirements and other artifacts with automated formalization \marco{This last part of the sentence should also be checked }  and integrating formal verifiers early.
\end{itemize}
\end{comment}


\subsection{Validity Risks}
\label{sec:validity1}
\pat{it should be useful to have risks discussed in just one place. Now they are discusses all around the paper. We can instead have a subsection of the research method or a section at the end of the paper.}

The following risks might exist in our study:
\begin{itemize}
    \item Our search string might miss relevant literature;
    \item The filtering using LLMs might have removed relevant literature, making our results incomplete;
    \item Our focus on certain conferences and journals might affect the outcome. Discussions about the future might also be present in other venues like dedicated workshops or seminars that our search strategy did not include;
    \item Sometimes, we had to interpret statements and map different wordings from different authors to consolidate the results from the literature study. Misinterpretation or misunderstanding might also influence the outcome.
\end{itemize}
